Computing large market equilibria using abstractions

Computing market equilibria is an important practical problem for market design, for example in fair division of items. However, computing equilibria requires large amounts of information (typically the valuation of every buyer for every item) and computing power. We consider ameliorating these issues by applying a method used for solving complex games: constructing a coarsened abstraction of a given market, solving for the equilibrium in the abstraction, and lifting the prices and allocations back to the original market. We show how to bound important quantities such as regret, envy, Nash social welfare, Pareto optimality, and maximin share/proportionality when the abstracted prices and allocations are used in place of the real equilibrium. We then study two abstraction methods of interest for practitioners: (1) filling in unknown valuations using techniques from matrix completion, (2) reducing the problem size by aggregating groups of buyers/items into smaller numbers of representative buyers/items and solving for equilibrium in this coarsened market. We find that in real data allocations/prices that are relatively close to equilibria can be computed from even very coarse abstractions.

==> approximation_results.tex <==
\section{Approximation Results}
We now look at how well properties of market equilibria are maintained in the equilibria derived from abstractions. We relate these quantities to various matrix norms of the error matrix $\Delta V$.  Individual bounds will largely be in terms of $\|\Delta v_i\|_1$, the $\ell_1$-norm of the change in values for buyer $i$. Bounds over all agents will mostly use the $\ell_1,\ell_{\infty}$-norm for matrices, but where the $\ell_1$ is applied to rows rather than columns: $$\|\Delta V\|_{1,\infty} = \max_{i \in [n]} \|\Delta v_i\|_1.$$
Note that the standard definition of this norm is to apply it to columns, not rows. Our definition can be thought of as the standard definition, but with a transpose applied before invoking the norm.

While this paper primarily focuses on the divisible setting, our results in this section all carry over to the indivisible setting.

\subsection{Individual optimality notions: envy, regret, and maximin share}
First we look at individual notions of optimality. These measures will compare how satisfied individuals are under their allocation $\hat{X}$. 

We begin with asking how well an equilibrium $(\hat{p}, \hat{X})$ represents buyers' true preferences. Although in many assignment problems prices are only `virtual' we can still judge the lifted equilibrium by using the abstracted price vector. One notion of how happy individuals are with their allocation $\hat{X}$ is the regret of the allocation. That is, how close is $\hat{x}_i$ to actually being a demand vector given the prices $\hat{p}$? Here we measure regret with respect to the supply constraints when the buyer can buy all items for themselves. Formally the regret of a buyer under a solution $(\hat{p}, \Xhat)$ is
\[\text{Regret}_i (\hat{p}, \hat{X}) = \max \{  u_i(x_i) : x_i\in \R^m_+, x_i \cdot \hat{p} \leq B_i, x_i \leq s\}  - u_i(\xhat_i).\]
By definition, in equilibrium, regret is $0$.

The envy for buyer $i$ is the amount by which they prefer any other buyers' allocation over their own. Equilibrium allocations are envy free in the equal-incomes setting where all buyers have the same budget. Envy is often used as a fairness metric in the fair-division setting~\citep{varian1974equity,budish2011combinatorial,caragiannis2016unreasonable}.
Formally, the envy is
\[\textrm{Envy}_i(\hat X) = \max_{i'\in [n]} u_i( \hat x_{i'}) - u_i(\hat x_i).\]
Note that the envy gap is zero in this definition, if buyer $i$ prefers their own bundle.

Finally, we look at a weak notion of fairness: the maximin share (MMS) guarantee. MMS is the value that buyer $i$ would obtain if they were allowed to split the allocation $X$ into $n$ bundles, but were then assigned their least-valued bundle $\min_{i'}u_i(x_{i'})$. MMS was introduced by \citet{budish2011combinatorial}, and it generalizes the \emph{proportional-share} notion of divisible assignment to the indivisible setting. In proportional-share assignment, each buyer $i$ is required to receive an allocation that they like at least as much as the one where they receive a fraction $\frac{1}{n}$ of each item. Since MMS generalizes fair share our result below applies to both fairness notions.

Formally, the MMS guarantee of buyer $i$ is
\[
  \textrm{MMS}_i = \max_{x \in X} \min_{i' \in [n]} u_i(x_{i'}).
\]

We say that the \emph{MMS gap} for buyer $i$ in allocation $x$ is
\[\textrm{MMS gap}_i(\Xhat)=\max (0, \textrm{MMS}_i - u_i(\xhat_i)).\]
The main result of this section shows that regret, envy, and MMS errors are bounded by the norm of the approximation error. All proofs can be found in the Appendix.

\begin{theorem}[Regret, Envy, MMS are linear in abstraction quality]
  \label{thm:approximate individual optimality}
The regret, envy, and MMS gap of buyer $i$ for any allocation $\Xhat$ under $\Vhat$ is maintained under $V$ up to individual additive error of $\|\Delta v_i\|_1$ for regret and envy, and $2\|\Delta v_i\|_1$ for the MMS gap. The maximum additive error over buyers is thus bounded by $\|\Delta V\|_{1,\infty}$.
\end{theorem}

\subsection{Global optimality notions: Pareto Optimality and Nash Social Welfare}
Often in market design the goal is to maximize social welfare, i.e., the sum of buyer utilities. However, in general, a market equilibrium may not lead to a social-welfare-maximizing solution. This is easy to see by considering the solution to the problem of maximizing geometric-mean utility: it is a market equilibrium, but it will never set any buyer utility to zero, even when that is  the only way to maximize social welfare. 

Instead, the usual efficiency criterion for market equilibria is that they are Pareto optimal (see e.g., \citet{varian1974equity,budish2011combinatorial,caragiannis2016unreasonable}). Nonetheless, Pareto optimality can be related to \emph{weighted} social welfare: Negishi's theorem~\citep{negishi1960welfare} says that given a market equilibrium, there exists a set of utility weights $\{\beta_i\}$ specifying the utility rate of each buyer such that the market-equilibrium allocation is the allocation that maximizes weighted social welfare. We can use this to show that a solution to $\Vhat$ approximately solves the weighted-social-welfare-maximization problem for a particular set of weights:

\begin{theorem}[Weighted social welfare is linear in abstraction quality]
  \label{thm:approximate negishi maximization}
  Let $\Xhat$ be the allocation of a market equilibrium for $\Vhat$, and $\{\beta_i\}$ the associated Negishi social-welfare weights. Then $\Xhat$ solves the problem of maximizing social welfare for $V$ under weights $\{\beta_i\}$ up to an additive error of at most $\|\beta\|_1\|\Delta V\|_{1,\infty}$.
\end{theorem}

Now we show that any Pareto-improving allocation has some buyer that does not gain much.

\begin{theorem}[Ability to Pareto improve is linear in abstraction quality]
  \label{thm:small strict pareto}
  Any Pareto-optimal solution under $\hat V$ is such that any Pareto-dominating allocation under $V$ has a buyer $i$ whose utility improves by at most $\| \Delta v_i \|_1$.
\end{theorem}

Theorems~\ref{thm:approximate negishi maximization} and~\ref{thm:small strict
  pareto} show that a solution $X$ computed for $\Vhat$ is approximately Pareto
optimal for $V$ in two senses: It approximately solves the weighted-welfare
maximization problem under the Negishi weights from $\Vhat$, and there is a
small amount of strong Pareto improvement. However, there is a third sense of
Pareto improvement which we cannot bound: there may be a Pareto improvement
where some buyer does not gain a lot, but the total improvement to (unweighted)
social welfare may be large. We call this largest improvement to unweighted
social welfare under any Pareto improvement the \emph{Pareto gap}.
Theorem~\ref{thm:approximate negishi maximization} guarantees that if the Pareto gap is large, then the large improvements will be for buyers with low
Negishi welfare weights, and thus they are, in a sense, buyers whose unweighted
utility should not be highly prioritized in market equilibrium.

So far we have discussed global optimality from the perspective of Pareto optimality. However, another global optimality condition that has gained recent interest from the perspective of fairness is Nash social welfare, which is deployed on Spliddit~\citep{caragiannis2016unreasonable}. The Nash social welfare (NSW) is the product of buyer utilities, formally
\[
  \text{NSW}(X) = \prod_{i\in [n]} u_i(x_i).
\]

We now show that NSW is also maintained up to multiplicative error in the approximation.  

\begin{theorem}[Nash Social Welfare is multiplicatively related to abstraction quality]
  \label{thm:nsw}
  The NSW of the optimal solution $\Xhat$ under $\Vhat$,  is bounded by the NSW of the optimal solution $X^*$ to the original problem as follows:
  \[
    \text{NSW}(X^*) \leq \prod_{i \in [n]}\bigg(1 +  \frac{\|\Delta v_i\|_1}{\hat u_i(x^*)}\bigg) \text{NSW}(\xhat).
  \]
  This assumes $\hat u_i(x^*_i)>0$ for all $i$, i.e., the difference between $V$ and $\Vhat$ should be such that the original optimal solution still has nonzero value under $\Vhat$.
\end{theorem}


% \begin{theorem}
%   The NSW of the approximate solution, $\hat u$ is bounded by the value of the optimal solution to the original problem $u^*$ as follows
%   \[
%     \hat u \geq \frac{u^*}{\bigg(1 + \sum_{S \subset [n]} \prod_{i \in S} \frac{\Delta u_i}{\hat u^*_i}\bigg)}
%   \]
% \end{theorem}
% \begin{proof}
%   Let $\hat{u}_i, u^*_i, \hat{u}^*_i$ be the utility of buyer $i$ in the optimal solution to the approximation, optimal solution to the original problem, and the value of the optimal solution to the original problem under the approximation. We let $\Delta u_i = u^*_i - \hat{u}^*_i$. We then have
%   \begin{align*}
%     u^* &= \prod_{i}u^*_i
%     = \prod_{i}(\hat u^*_i + \Delta u_i)
%     = \prod_{i} \hat u^*_i + \sum_{S \subset [n]} \prod_{i \in S} \Delta u_i \prod_{i \notin S} \hat u^*_i
%     = \prod_{i} \hat u^*_i + \sum_{S \subset [n]} \prod_{i \in S} \frac{\Delta u_i}{\hat u^*_i} \prod_{i \in [n]} \hat u^*_i \\
%     &= \bigg(1 + \sum_{S \subset [n]} \prod_{i \in S} \frac{\Delta u_i}{\hat u^*_i}\bigg) \hat u^*
%     \leq \bigg(1 + \sum_{S \subset [n]} \prod_{i \in S} \frac{\Delta u_i}{\hat u^*_i}\bigg) \hat u
%   \end{align*}
% \end{proof}

Note that the theorem also implies a bound for the geometric mean of the buyer utilities, which is the n'th root of the NSW.





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> convex_program.tex <==
\section{Convex Program}

To compute a market equilibrium for either a full market or an abstracted market we use the celebrated Eisenberg-Gale convex program, which computes a market equilibrium in a linear Fisher market~\citep{eisenberg1959consensus}.

\citet{cole2017convex} give the following primal convex program (as well as a
dual not included here) for computing a solution to a Fisher market with
quasi-linear utilities. 
%We denote the primal convex program by {\mcp}.

\small
\noindent\begin{minipage}{.55\linewidth}
\begin{equation}
  \begin{gathered}
    \max_{x\geq 0,\delta \geq 0, u} \quad \sum_{i} B_i\log(u_i) - \delta_i \nonumber\\
    u_i \leq \sum_j x_{ij} v_{ij} + \delta_i, \forall i  \\
    \sum_i x_{ij} \leq 1, \forall j  
    %x_{ij},\delta_i  \geq 0\nonumber
  \end{gathered} \label{eq:cp_max_primal}
  %\vspace{-1.5mm}
\end{equation}
\end{minipage}
\noindent\begin{minipage}{.48\linewidth}
\begin{equation}
  \begin{gathered}
    \min_{p,\beta} \quad \sum_{j} p_j - \sum_i B_i\log(\beta_i) \\
    \forall i, p_j \geq v_{ij}\beta_i \\
    \beta_i  \leq 1
  \end{gathered} \label{eq:cp_max_dual}
  %\vspace{-1.5mm}
\end{equation}
\end{minipage}
\normalsize

The variables $x_{ij}$ denote the amount of item $j$ that bidder $i$ receives,
$\delta_i$ being nonzero denotes bidder $i$ saving some of their budget, and
$u_i$ denotes a measure of utility for bidder $i$ (exactly their utility when
$\delta_i=0$, otherwise it is not exact).

The dual variables $\beta_i, p_j$ correspond to the first and second
constraints, respectively. They can be interpreted as follows: $\beta_i$ is the
inverse bang-per-buck: $\min_{j:x_{ij}>0}\frac{p_j}{v_{ij}}$ for buyer $i$, and
$p_j$ is the price of good $j$.

The leftover budget is denoted by $\delta_i$, it arises from the dual program:
it is the dual variable for the dual constraint $\beta_i \leq 1$, which
constrains bidder $i$ to paying at most a cost-per-utility rate of $1$. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> def.tex <==
% From Christian

\newcommand{\Vhat}{\ensuremath{\hat{V}}}
\newcommand{\Vclustered}{\ensuremath{\tilde{V}}}
\newcommand{\xhat}{\ensuremath{\hat{x}}}
\newcommand{\phat}{\ensuremath{\hat{p}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math environments, get defined if they do not already exist
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{etoolbox}
\ifcsmacro{assumption}{}{
	\newtheorem{assumption}{Assumption}[]
}
\ifcsmacro{corollary}{}{
	\newtheorem{corollary}{Corollary}[]
}
\ifcsmacro{definition}{}{
	\newtheorem{definition}{Definition}[]
}
\ifcsmacro{example}{}{
	\newtheorem{example}{Example}[]
}
\ifcsmacro{fact}{}{
	\newtheorem{fact}{Fact}[]
}
% \ifcsmacro{lemma}{}{
% 	\newtheorem{lemma}{Lemma}[]
% }
\ifcsmacro{proposition}{}{
	\newtheorem{proposition}{Proposition}[]
}
\ifcsmacro{remark}{}{
	\newtheorem{remark}{Remark}[]
}
\ifcsmacro{theorem}{}{
	\newtheorem{theorem}{Theorem}[]
}

\ifcsmacro{lemma}{}{
	\newtheorem{lemma}{Lemma}[]
}
% Make := and =:
\usepackage{mathtools}
\mathtoolsset{centercolon}
\newcommand{\defeq}{\mathrel{:\mkern-0.25mu=}}
\newcommand{\eqdef}{\mathrel{=\mkern-0.25mu:}}

\newcommand\defeqq{\stackrel{\mathclap{\normalfont\mbox{def}}}{=}}
\newcommand{\epsne}{$\epsilon$-Nash equilibrium}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\eps}{\epsilon}

\newcommand{\bbB}{\ensuremath{\mathbb{B}}}
\newcommand{\bbD}{\ensuremath{\mathbb{D}}}
\newcommand{\bbE}{\ensuremath{\mathbb{E}}}
\newcommand{\bbI}{\ensuremath{\mathbb{I}}}
\newcommand{\bbN}{\ensuremath{\mathbb{N}}}
\newcommand{\bbR}{\ensuremath{\mathbb{R}}}
\newcommand{\bbS}{\ensuremath{\mathbb{S}}}

\newcommand{\Rplus}{\ensuremath{\mathbb{R}_+}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}


\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\cfr}{CFR}
\newcommand{\cfrp}{CFR$^+$}
\newcommand{\rmp}{RM$^+$}
\newcommand{\mccfr}{MCCFR}
\newcommand{\egt}{EGT}
\newcommand{\mdescent}{MD}
\newcommand{\mprox}{MP}
\newcommand{\smprox}{SMP}

\def\prox{\mathop{\rm Prox}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Game theory definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\epsnash}{\ensuremath{{\epsilon}}-Nash equilibrium}
\newcommand{\nash}{NE}
\newcommand{\cfrstrat}{BCR}
\newcommand{\crswf}{CRSWF}
\newcommand{\epsilonsad}{{\epsilon_{\hbox{\scriptsize\rm sad}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Misc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\todo}[1]{{\color{blue} #1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% From Fatma

\def\crd{\color{red}}
\def\cbl{\color{blue}}
\def\cgr{\color{green}}
\def\cmg{\color{magenta}}

\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}[1]{\label{#1}\end{eqnarray}}
\newcommand{\nn}{\nonumber \\}
	\newcommand{\ese}{\end{eqnarray*}}
	\newcommand{\bse}{\begin{eqnarray*}}
	\def\beq{\begin{equation}}
	\def\eeq{\end{equation}}
	\def\Bbb#1{{\bf #1}}
	\def\eqnum#1{\eqno (#1)}
	\def\fnote#1{\footnote}
	
	\def\ra{\rangle}
	\def\la{\langle}
	\def\ul{\underline}
	\def\*{{{\LARGE\bf $^*$}}}
	\def\P{{{\LARGE\bf $^+$}}}
	\def\PP{{{\LARGE\bf $^{++}$}}}
	
	\def\P{{\textsf\bf P\,}}
	\def\NP{{\textsf\bf NP\,}}
	
	\def\N{{\mathbb{N}}}
	\def\R{{\mathbb{R}}}
	\def\Z{{\mathbb{Z}}}
	
	\def\mones{{\mathbf{1}}}
	
	\def\bA{{\mathbf{A}}}
	\def\bB{{\mathbf{B}}}
	\def\bC{{\mathbf{C}}}
	\def\bD{{\mathbf{D}}}
	\def\bE{{\mathbf{E}}}
	\def\bF{{\mathbf{F}}}
	\def\bG{{\mathbf{G}}}
	\def\bH{{\mathbf{H}}}
	\def\bI{{\mathbf{I}}}
	\def\bJ{{\mathbf{J}}}
	\def\bK{{\mathbf{K}}}
	\def\bL{{\mathbf{L}}}
	\def\bM{{\mathbf{M}}}
	\def\bN{{\mathbf{N}}}
	\def\bO{{\mathbf{O}}}
	\def\bP{{\mathbf{P}}}
	\def\bQ{{\mathbf{Q}}}
	\def\bR{{\mathbf{R}}}
	\def\bS{{\mathbf{S}}}
	\def\bT{{\mathbf{T}}}
	\def\bU{{\mathbf{U}}}
	\def\bV{{\mathbf{V}}}
	\def\bW{{\mathbf{W}}}
	\def\bX{{\mathbf{X}}}
	\def\bY{{\mathbf{Y}}}
	\def\bZ{{\mathbf{Z}}}
	
	
	
	\def\cA{{\cal A}}
	\def\cB{{\cal B}}
	\def\cC{{\cal C}}
	\def\cD{{\cal D}}
	\def\cE{{\cal E}}
	\def\cF{{\cal F}}
	\def\cG{{\cal G}}
	\def\cH{{\cal H}}
	
	\def\cJ{{\cal J}}
	\def\cK{{\cal K}}
	\def\cL{{\cal L}}
	\def\cM{{\cal M}}
	\def\cN{{\cal N}}
	\def\cO{{\cal O}}
	\def\cP{{\cal P}}
	\def\cQ{{\cal Q}}
	\def\cR{{\cal R}}
	\def\cS{{\cal S}}
	\def\cT{{\cal T}}
	\def\cU{{\cal U}}
	\def\cV{{\cal V}}
	\def\cW{{\cal W}}
	\def\cX{{\cal X}}
	\def\cY{{\cal Y}}
	
	
	\def\Ic{{\overline{I}}}
	
	%\def\e{\mathop{{\rm e}}}
	%\def\i{{\mathop{z}}}
	\def\nrm{\mathop{{\parallel}}}
	\def\vrt{\mathop{\,\mid}\,}
	\def\eqbd{\colon =}
	
	\def\Opt{{\hbox{\rm Opt}}}
	\def\Argmin{\mathop{\rm Argmin}}
	\def\argmin{\mathop{\rm argmin}}
	\def\Argmax{\mathop{\rm Argmax}}
	\def\argmax{{\mathop{\rm argmax}}}
	
	\def\Sad{{\mathop{\rm Sad}}}
	\def\Residual{\mathop{{\rm Residual}}}
	\def\DualityGap{{\hbox{\rm DualityGap}}}
	
	\def\sign{\mathop{{\rm sign}}}
	\def\sgn {{\rm \,sgn}}
	\def\const{{\hbox{\rm const}}}
	\def\Card{{{\mathop{\rm Card}}}}
	\def\card{\mathop{\rm card}}
	\def\data{\hbox{\rm data}}
	\def\Supp{{\hbox{\rm Supp}}}
	\def\nnz{{\hbox{\rm nnz}}}
	\def\Size{\mathop{{\rm Size}}}
	\def\size{\mathop{{\rm Size}}}
	\def\Sz{\mathop{{\hbox{\sl Size}}}}
	\def\Diam{\mathop{{\rm Diam}}}
	\def\AvDiam{\mathop{{\rm AvDiam}}}
	\def\Vl{\mathop{{\hbox{\sl Vol}}}}
	\def\Vol{\mathop{{\rm Vol}}}
	\def\vol{\mathop{{\rm vol}}}
	
	\def\rank{\mathop{\rm Rank}}
	\def\Diag{\mathop{{\rm Diag}}}
	\def\diag{{\rm diag}}
	\def\trace{{\rm Trace}}
	\def\Tr{\mathop{{\rm Tr}}}
	\def\Det{\mathop{{\rm Det}}}
	\def\Fr{{\hbox{\scriptsize Fr}}}
	\def\Arrow{{\hbox{\rm Arrow}}}
	\def\Col{{\hbox{\rm Col}}}
	\def\Row{{\hbox{\rm Row}}}
	
	\def\Prob{{\hbox{\rm Prob}}}
	\def\Cov{{\hbox{\rm Cov}}}
	\def\uniform{\mathop{\rm uniform}}
	
	\def\dim{\mathop{{\rm dim}\,}}
	\def\codim{\mathop{{\rm codim\,}}}
	\def\Lin{{\mathop{\rm Lin}}}
	\def\lin{{\mathop{\rm lin}}}
	\def\Aff{{\mathop{\rm Aff}}}
	\def\aff{{\mathop{\rm aff}}}
	\def\vspan{{\mathop{\rm span}}}
	\def\intt{{\mathop{\rm int}\,}}
	\def\inter{\mathop{{\rm int}}}
	\def\rint{{\mathop{\rm rint\,}}}
	\def\ri{{\mathop{\rm ri}\,}}
	\def\partialri{\mathop{\partial_{\rm ri}}}
	\def\cl{{\mathop{\rm cl}\,}}
	\def\closure{{\rm cl}}
	\def\bd{{\mathop{\rm bd}\,}}
	\def\rbd{{\mathop{\rm rbd}\,}}
	
	
	\def\Dom{\mathop{{\rm Dom}}}
	\def\dom{{\mathop{\rm dom}}}
	\def\Epi{{\mathop{\rm Epi}}}
	\def\epi{{\rm epi}}
	
	\def\Ker{\mathop{{\rm Ker}}}
	\def\ker{\mathop{{\rm Ker}}}
	\def\Image{\mathop{{\rm Im}}}
	\def\Conv{{\mathop{\rm Conv}}}
	\def\conv{\mathop{{\rm Conv}}}
	\def\co{\mathop{{\rm Conv}}}
	\def\Cone{{\mathop{{\rm Cone\,}}}}
	\def\cone{\mathop{{\rm Cone}}}
	\def\Ext{{\mathop{\rm Ext}}}
	\def\Extr{{\mathop{\rm Extr}}}
	\def\Rec{{\mathop{{\rm Rec}}}}
	\def\rec{{\mathop{{\rm Rec}}}}
	
	\def\dist{\mathop{{\rm dist}}}
	\def\log{\mathop{{\rm log}}}
	\def\asin{{\hbox{\rm asin}}}
	\def\Polar{{\mathop{{\rm Polar\,}}}}
	\def\ch{{\mathop{\rm ch\,}}}
	\def\arc{{\mathop{\rm arc\,}}}
	\def\EllIn{{\mathop{\rm EllIn}}}
	\def\GDA{{\rm \ ArD\ }}
	\def\GDS{{\rm \ StD\ }}
	\def\lev{{\mathop{\rm lev}}}
	
	\def\CE{\mathop{{\hbox{\sl CircEll}}}}
	\def\CS{\mathop{{\hbox{\sl CircSimp}}}}
	\def\IE{\mathop{{\hbox{\sl InscrEll}}}}
	\def\Compl{\mathop{{\rm Compl}}}
	\def\Accur{\mathop{{\rm Accur}}}
	\def\mes{\mathop{{\rm mes}}}
	\def\EllOut{\mathop{{\rm EllOut}}}
	\def\Ell{\mathop{{\sl Ell}}}
	\def\InnerRad{\mathop{{\rm InnerRad}}}
	\def\Mom{\mathop{\rm Mom}}
	\def\Loss{{\hbox{\rm Loss}}}
	
	
	\def\huh{\hbox{\vrule width 2pt height 8pt depth 2pt}}
	
	\def\rdiamondsuit{{\color{red}$\diamondsuit$}}
	\def\blacksquare{\hbox{\vrule width 4pt height 4pt depth 0pt}}
	\def\square{\hbox{\vrule\vbox{\hrule\phantom{o}\hrule}\vrule}}
	
	
	\def\nr{\par \noindent}
	\def\pn{\par\noindent}
	\def\qr{\qquad\cr}
	\def\fig{\epsfxsize=220pt\epsfysize=140pt\epsffile}
	\def\mypictsmall{\epsfxsize=120pt\epsfysize=120pt\epsffile}
	\def\mypictvsmall{\epsfxsize=90pt\epsfysize=90pt\epsffile}
	
	\def\bStnu{\bS^{\widetilde{\nu}}}
	\def\bStnup{\bS^{\widetilde{\nu}}_+}
	
	


==> quasilinear_results.tex <==

\section{Efficiency Bounds for the Quasi-Linear Setting}

\subsection*{Regret Bound}
First we show how to bound the regret associated with each buyer. Say that
$x_i^*$ is the optimal allocation for buyer $i$ under $V$ and prices $p$. Since
$\xhat^*_i$ is optimal under $\Vhat$ we have
\[
  (\Vhat_i - \phat) \xhat^*_i \geq (\Vhat_i - \phat) x^*_i
  \Rightarrow 
  (V_i + \Delta V_i - \phat) \xhat^*_i \geq (V_i + \Delta V_i - \phat) x^*_i,
\]
and thus the regret is bounded by $\Delta V_i (x^*_i-\xhat^*_i)$. Now we can
sum over all bidders to get
\begin{align}
  \sum_{i\in N} r_i \leq \sum_{i \in N} \langle \Delta V_i, x^*_i-\xhat^*_i  \rangle
  = \sum_{j \in M} \sum_{i \in N} \Delta V_{ij} (x^*_{ij} -\xhat^*_{ij})
  = \sum_{j \in M} \langle \Delta V_{j}, x^*_{j} -\xhat^*_{j} \rangle.
  % \leq \sum_{j \in M} 2\max_{i} |\Delta V_{ij}|
  \label{eq:regret inner product bound}
\end{align}

We now have a few options on how to bound \eqref{eq:regret inner product bound}.
% First we give a bound based on the Frobenius norm:
% \begin{align}
%   \eqref{eq:regret inner product bound}
%   \leq \sum_{j \in M} \| \Delta V_j \|_2 \| x_j^* - \xhat^*_j \|_2
%   \leq 2\sqrt{n}\sum_{j \in M} \| \Delta V_j \|_2
%   \leq 2\sqrt{nm} \| \Delta V \|_F.
% \end{align}

First we give a bound based on the $\ell_\infty,\ell_1$ matrix norm:
\begin{align}
  \eqref{eq:regret inner product bound}
  \leq 2 \sum_{j\in M} \max_{j\in N} \Delta V_{ij}
  \leq 2 \sum_{j\in M} \|\Delta V_{j} \|_{\infty}
  = 2 \| \Delta V \|_{\infty, 1}
  \label{eq:regret bound infty one norm}
\end{align}

Based on \eqref{eq:regret bound infty one norm} we can get a (looser) bound for
the Frobenius norm:
\begin{align}
  \eqref{eq:regret bound infty one norm}
  \leq 2\sqrt{m} \| \Delta V \|_{F}
  \label{eq:regret bound frobenius}
\end{align}

\subsection{Core property}
As shown by \citet{conitzer2019pacing}, the equal-rates market equilibrium corresponds to a first-price pacing equilibrium. In this setting we care not only about the utility of the buyers, but also the revenue of the seller. \citet{conitzer2019pacing} show that FPPE are in the core. We show that this property is approximately preserved:
\begin{theorem}
  [Approximately in the core]
  Any market equilibrium with respect to $\hat V$ is in the $\|\Delta V\|_{1, \infty}$-core with respect to $V$.
\end{theorem}
\begin{proof}
  Let S be a subset of buyers that have a dominant allocation $x,\delta$ such that every buyer is weakly better off under $V$ and the seller makes weakly more money. We know that $\hat x, \hat \delta$ is in the core for $\hat V$, so some bidder satisfies
  
  \[
    \langle \hat v_i, \hat x_i \rangle + \hat \delta
    > \langle \hat v_i, x_i \rangle + \delta
    = \langle v_i - \Delta v_i, x_i \rangle + \delta
    \geq \langle v_i , x_i \rangle - \| \Delta v_i \|_1 + \delta
  \]
  So,
  \[
    \langle v_i , x_i \rangle + \delta
    \leq \langle \hat v_i , \hat x \rangle + \hat \delta + \| \Delta v_i \|_1
  \]
\end{proof}

\section{Counterexamples}

The following example shows that in the setting where we use the approximation to compute posted prices the efficiency and revenue loss can be complete: neither  buyer wants any item, even at a fairly low amount of error.
\begin{example}
  There are 2 bidders and 1 good. Each bidder has valuation and budget of
  one. Now consider an approximate instance with valuations $1+\epsilon$. In the
  approximate instance, the equilibrium price is $1+\epsilon$, with any full
  allocation legal, since the buyers are then indifferent. If we implement this
  price in the original instance then neither buyer wants the item, and
  revenue and social welfare is zero.
\end{example}

The following instance from \citet{conitzer2019pacing} shows that a small change in value for a bidder can lead to large overall social welfare loss. Note that this example only works in the quasi-linear setting; if money has no intrinsic value then value changes do not matter in this example, since the price gets set to $2.5$ no matter what.
\begin{example}
	There are 2 bidders, 1 good. We have values $v_{11} = K, v_{21} = 1$, and budgets $B_1 = \frac12, B_2 = 2$. The FPPE is $a_1 = \frac1K, a_2 = 1$ and $x_{11} = x_{21} = \frac12$, for total social welfare $\frac{k+1}2$. Now increase $v'_{21} = 2$. The new FPPE will have $a_1 = \frac2K, a_2 = 1$, and $x_{11} = \frac14, x_{21} = \frac34$ for social welfare of $\frac{k+3}{4}$, as $K\rightarrow \infty$ we lose $\frac12$ of the social welfare.
\end{example}


==> recursive_market_equilibrium.tex <==
\section{Recursive Lift}

The simplest procedure for lifting the solution from the representative market to the original is to divide the allocations of each representative buyer among the original buyers allocations proportional to their share of the representative-buyer budget. This allowed us to give theoretical results on solution quality using our framework of measuring matrix distances. 

However, we now consider another candidate lift. First, let us define $x^{R}$ to be an allocation of original items to representative buyers. We define a lift $L(x^{R})$ to be an allocation to the original buyers such that they are only allocated items from their respective representative buyer. We let $L_i(x^{R})$ be the bundle of goods received by buyer $i$ in the lift. We denote by $R_{\tilde i}$ the set of buyers assigned to representative buyer $\tilde i$.

\begin{defn}
  $L(x^R)$ is a \textit{local lift} if for any representative buyer $\tilde i$, we have that $\sum_{i \in R_{\tilde i}} L_i(x^R) \leq x^R_{\tilde i}$.
\end{defn}

Secondly, we shall use the less formal restriction that a local lift should be computable using only $x^R$ and the set of valuations $\{v_i : i \in R_{\tilde i}\}$. 

The concept of a local lift is natural when we want to consider using parallelization for the computation of the lift. Locality means that only information about the allocation a representative buyer received is used to compute the re-allocation to the buyers represented by the representative buyer. Thus, we can solve the main abstraction and then solve each component of the lift (defined by each representative buyer) in parallel without any message passing. The proportional lift is a local lift.

Recall that the original objective function for the EG equilibrium is the maximization of Nash social welfare. Thus, we now consider a lift which we will show is optimal in the family of local lifts in the sense that it is the NSW-maximizing one.

The lift works as follows:
For each representative buyer, we look at the allocation of original items to that representative buyer in the abstraction equilibrium, denote this by $\tilde{x}^R_{\tilde i}$. We then construct a new \emph{local} market for each representative buyer $i$. The buyers in the local market are individuals in $R_{\tilde i}$, their budgets are their original budgets, and supplies are $\tilde{x}^R_{\tilde i}$. 

The lift $L(x^R)$ is the solution to $$\max_{x} \sum_{i \in R_{\tilde i}} \text{log} v_i \cdot x_i \text{ s.t. } \sum_{i \in R_{\tilde i}}{x_i} \leq \tilde{x}^{R}_{\tilde i} .$$
Which yields a market equilibrium in the local market. We call this approach \emph{recursive market equilibrium} (RME). From the way the lift is construct it is obvious that:

\begin{theorem}
  A local lift maximizes Nash social welfare among all local lifts if and only if it is an RME.
\end{theorem}

We can also show that RME is guaranteed to improve on several metrics relative to the proportional lift: Pareto gap, regret, MMS gap, and (by the above Theorem) NSW. Intuitively, this is due to the utility guarantee provided by market equilibrium, which says that each buyer does better than their budget-proportional allocation of each item.

\begin{theorem}
  Let $x,p$ be a solution obtained from proportional allocation from solving a representative market instance. Let $x^r,p$ be the solution obtained by applying  RME to $x,p$. The RME solution leads to weakly lower Pareto gap, regret, and MMS gap, as well as weakly higher NSW.
  \label{thm:recursive_objectives}
\end{theorem}
\begin{proof}

First we note the following simple fact which holds for any agent $i$: the utility of $i$ under $x^r$ is weakly greater than that under $x$, i.e., $\langle  v_i, x^r_i \rangle \geq \langle  v_i, x_i \rangle$. This is because (a subset of) $x^r$ is a market equilibrium in the recursive market for the corresponding $\tilde i$, and an agent is guaranteed to get at least the value of the budget-proportional allocation in any market equilibrium.

  The Pareto gap is the value of a linear program that maximizes social welfare (minus current welfare) subject to the constraint that each agent is weakly better off. Since utilities are greater in $x^r$ this is a strictly more constrained problem than for $x$, and thus the value, i.e., the Pareto gap, is lower.

  Since we keep prices the same the optimal bundle $x_i^*$ for each agent remains the same for $(x,p)$ and $(x^r,p)$. Thus the only affected part of regret is the negative term, which is weakly greater under $x^r$ since utilities are weakly greater.

  That the MMS gap is smaller and NSW greater follows directly from each agent having weakly-higher utility.
\end{proof}


While the objectives in Theorem~\ref{thm:recursive_objectives} are all guaranteed to improve, the below example shows that envy might be higher under the RME than the proportional lift. Intuitively, this is because in we may have an agent $i$ who does not envy agent $j$ very much in the proportional lift, but in the RME $j$'s lot improves very much while $i$'s improves very little, thus generating an increase in envy. 

\begin{example}
  Consider a 5-buyer-4-item instance with valuations $v_1=v_2=[1.5,1.5,0,0], v_3=[0,0,1+\eps,1-\eps], v_4=[0,0,1-\eps,1+\eps], v_5=[1.5,1.5,1+\eps,1-\eps]$ and budgets of $1$. Now consider the abstraction where buyers $1,2,5$ are clustered to a representative buyer with valuation $v_{\tilde 1}=[1.5,1.5,0,0]$ and budget $3$, and buyers $3,4$ are clustered to a representative buyer with valuation $v_{\tilde 2}=[0,0,1.5,1.5]$ and budget $2$. The representative market equilibrium with equal rates is to assign representative buyer $\tilde 1$ all of items $1$ and $2$, each with price $1.5$ and assign representative buyer $\tilde 2$ all of $3$ and $4$ at price $1$ each. This assignment leads to no envy when we perform the budget-proportional allocation. However, if we apply RME to representative buyer $\tilde 2$ then buyers $3$ and $4$ get assigned all of items $3$ and $4$, respectively. Now buyer $5$ envies buyer $3$, as they could get $\eps$ more utility.
\end{example}

We view the potential increase in envy as a necessary price to pay in order to reap the benefits of locally optimizing each of the representative allocations. In order to avoid potential envy increases, we would need to take into account agents $i \notin R_{\tilde i}$ when computing the lift, which would often not be feasible computationally (since the whole point of the representative abstraction was to avoid a convex program whose size is on the order of $n \times m$).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

